Non-myopic Generation of Language Models for Reasoning and Planning

Large Language Models have demonstrated remarkable abilities in reasoning and planning by breaking down complex problems into sequential steps. Despite their success in various domains like mathematical problem-solving and coding, LLMs face challenges in ensuring reliable and optimal planning due to their inherent myopic nature of autoregressive decoding. This paper revisits LLM reasoning from an optimal-control perspective, proposing a novel method, Predictive-Decoding, that leverages Model Predictive Control to enhance planning accuracy. By re-weighting LLM distributions based on foresight trajectories, Predictive-Decoding aims to mitigate early errors and promote non-myopic planning. Our experiments show significant improvements in a wide range of tasks for math, coding, and agents. Furthermore, Predictive-Decoding demonstrates computational efficiency, outperforming search baselines with reduced computational resources. This study provides insights into optimizing LLM planning capabilities.

==> paragraphs/01_abstract.tex <==
Large Language Models have demonstrated remarkable abilities in reasoning and planning by breaking down complex problems into sequential steps. Despite their success in various domains like mathematical problem-solving and coding, LLMs face challenges in ensuring reliable and optimal planning due to their inherent myopic nature of autoregressive decoding. This paper revisits LLM reasoning from an optimal-control perspective, proposing a novel method, \methodname{}, that leverages Model Predictive Control to enhance planning accuracy. By re-weighting LLM distributions based on foresight trajectories, \methodname{} aims to mitigate early errors and promote non-myopic planning. Our experiments show significant improvements in a wide range of tasks for math, coding, and agents. Furthermore, \methodname{} demonstrates computational efficiency, outperforming search baselines with reduced computational resources. This study provides insights into optimizing LLM planning capabilities. Code is available in this \href{https://anonymous.4open.science/r/Anonymous-20F2}{anonymous repo}.


==> paragraphs/06_discussion.tex <==
\paragraph{}

==> paragraphs/08_theory.tex <==
Recall that \methodname{} samples from a distribution to solve the trajectory optimization problem using LLM evaluation as the proxy for calculating future return. Similarly we can define such distribution for any trajectory-wise target. 

\begin{proposition} Let $\mathcal{J}$ be the target of trajectory optimization, and each step of trajectory should be generated causally with large language model $a_t \sim P^{\text{LLM}}\left(a_t\mid \mathbf{a}_{<t}, \mathbf{s}_{<t}\right)$ and the support set of this distribution is $\mathcal{P}$. Then the distribution that solves the optimization problem : 
\begin{equation}
    p(a_t)\propto P^{\text{LLM}}\left(a_t\mid \mathbf{a}_{<t}, \mathbf{s}_{<t}\right)\exp\left[ \mathbb{E}_{\mathbf{a}_{>t}}\mathcal{J}\left(\mathbf{s}_0;\mathbf{a}_{0:T}\right )\right]
\end{equation}
\end{proposition}

This form follows that of energy based model where the distribution $p(x)=\exp \left\{\sum_i \mu_i f_i(\mathbf{x})\right\} / Z $ minimizes the energy function $E^{\mu}(x):=-\sum_i\mu_if_i(x)$. We could use the same sampling technique to minimize the energy function $E = -\mathcal{J}$ left to right, achieving global-optimal planning. 

Here we study left-to-right planning by minimizing different forms of energy landscapes. Apart from the non-myopic LLM evaluation with foresight as introduced in \S\ref{sec: predictive decoding}, we study two types of energy functions: (1) Heuristic Functions and (2) Outcome Reward Models (ORM). Heuristic functions can be seen as human designed objectives that could act as guide for planning. ORMs assign confidence to reasoning chain and act as a verifier for the entire generation. Both types of function could be used to evaluate sampled foresights and reshape the generation distribution. 

\paragraph{Guiding Agent Planning with Heuristics} In this section, we use simple designed energy functions to guide LLM planning $E(\tau)$. We follow \citet{ma2024agentboard} using a simple matching function between intermediate states and the goal state as a heuristic function. The energy function is sparse such that more than one step need to be taken in order to achieve progress. 

\input{tables/agent_function}


\paragraph{Guiding Agent Planning with ORM} ORMs are easy to obtain, in contrast progress reward models (PRM) are difficult to train without expert annotation~\citep{wang2023math, lightman2023let}. Currently LLMs are limited by the scarce of trajectory-level optimization method and often relies on PRM to improve performance at inference time. Here we also compare with Monte Carlo Tree Search, which also does not need step level supervision. 

\input{tables/orm}




==> tables/myopia.tex <==
\begin{table}[ht!]
\centering
\caption{Myopic Gap Statistics of Llama3-8B model on GSM8K and MATH, using Beam Search and Predictive Decoding as reference.\jh{This table is hard to read, because these numbers are not really that interpretable without references. Like what does 0.03 mean? is that a large gap or small gap? we have no clues.}}
\resizebox{0.98\linewidth}{!}{
\begin{tabular}{ccccccc}
\toprule
\multirow{2}{*}{Task} & Mean $p^*$  & Mean $p^*$  & Mean $p^*$  & \multirow{2}{*}{$p^*>0.01$} & \multirow{2}{*}{$p^*>0.05$} & \multirow{2}{*}{$p^*>0.1$} \\ & (Beam Search) & (Predictive Decoding) & (Combined)\\
\midrule
\gsm &        0.029             &         0.059                                    &      0.070             &       59.2\%               &       41.0\%               &            24.3\%         \\ \matheval
 &      0.030              &    0.025                        &   0.032               &       62.9\%            &     17.4\%                 &     4.8\%         
\\
\bottomrule
\end{tabular}
}
\label{tab: myopic stats}
\end{table}
